Towards a HIPAA Compliant Agentic AI System in Healthcare

Agentic AI systems powered by Large Language Models (LLMs) as their foundational reasoning engine, are transforming clinical workflows such as medical report generation and clinical summarization by autonomously analyzing sensitive healthcare data and executing decisions with minimal human oversight. However, their adoption demands strict compliance with regulatory frameworks such as Health Insurance Portability and Accountability Act (HIPAA), particularly when handling Protected Health Information (PHI). This work-in-progress paper introduces a HIPAA-compliant Agentic AI framework that enforces regulatory compliance through dynamic, context-aware policy enforcement. Our framework integrates three core mechanisms: (1) Attribute-Based Access Control (ABAC) for granular PHI governance, (2) a hybrid PHI sanitization pipeline combining regex patterns and BERT-based model to minimize leakage, and (3) immutable audit trails for compliance verification.

==> oldfile.tex <==

% A core requirement for HIPAA compliance is the ability to audit data flows, detect unauthorized access, and produce evidence if a breach occurs. The audit \& monitoring modul implements a two-tier logging strategy such as \textit{interaction logging} and \textit{PDP decision logs}. The former logs the sanitized user queries, policy decisions, and any redaction operations. This log is stored in an encrypted database with access restricted to compliance officers or other authorized roles. If the LLM output was redacted, we store both the ``raw'' version from the LLM and the ``sanitized'' version delivered to the user, ensuring forensic traceability. The latter writes each allow/deny decision to an immutable ledger. This ledger, which is backed by a secure event log, helps detect tampering and provides verifiable proof of enforcement.



% For example, accessing patient records is only permitted during business hours (8AM-6PM) and from within the hospital's secure network. Access attempts outside these conditions are automatically denied. 


% We define policies in machine-readable form, such as an XACML-like syntax that captures who (role, identity, or attribute) can access what (specific types of PHI or data fields) under which conditions (context, time, obligations). An example of a simplified role-based physician access policy is illustrated in Fig. \ref{fig:physician_access}. The Policy Enforcement Point (PEP) serves as the gatekeeper in our system, intercepting access requests, and enforcing decisions rendered by the Policy Decision Point (PDP). Positioned at the boundary between users and protected resources, the PEP collects request attributes (e.g., user identity, resource identifier, and action) and forwards them to the PDP for evaluation.
% \begin{figure}[H]
% %\vspace{-2mm}
%     \centering 
%     \begin{minipage}{8.4cm}
%         \begin{tcolorbox}[enhanced,attach boxed title to top center={yshift=-1mm,yshifttext=-1mm},
%             colback=blue!10!white,colframe=gray!90!black,colbacktitle=gray!80!black, left=0.1mm, right=0.5mm, boxrule=0.50pt]
%             \footnotesize
%             {\fontfamily{cmr}\selectfont
%            \texttt{Policy: \\{"subjects": ["Physician"],
%            \\"resources": ["PHI.PatientName", "PHI.DOB", "PHI.Medications"],
%            \\"actions": ["read", "query"],
%            \\"conditions": ["consentGranted", "treatmentContext"],
%            \\"obligations": ["logAccess", "redactIdentifiers"]}}
%             }
%         \end{tcolorbox}
%     \end{minipage}    
%     \caption{An example Physician (role) access policy.}
%    %\vspace{-4mm}
%     \label{fig:physician_access}
%   %\vspace{-3mm}
% \end{figure}


% \begin{algorithm}
% \caption{UCON\textsubscript{\textit{ABC}} Policy Decision Workflow}
% \label{alg:pdp}
% \begin{algorithmic}[1]
% \Require Subject \(s\), Object \(o\), Action \(action\), Context \(ctx\), Session State \(S_t\)
% \Ensure Decision \{ALLOW, DENY\}, Updated \(S_t\)
% \Statex
% \Function{EvaluateRequest}{$s, o, action, ctx, S_t$}
%     \State $policies \gets \text{LoadPolicies}()$
%     \State $\text{Sort}(policies, \text{priority})$ \Comment{Priority: e.g., role-specific first}
%     \For{$policy \in policies$}
%         \If{\textbf{not} \Call{MatchSubjectAttributes}{$s, policy.A_s$}} 
%             \Continue \Comment{Skip non-matching policies}
%         \EndIf
%         \If{\textbf{not} \Call{MatchObjectAttributes}{$o, policy.A_o$}}
%             \Continue
%         \EndIf
%         \If{\textbf{not} \Call{CheckConditions}{$ctx, policy.C$} \textbf{or} $S_t.\text{phi\_count} \geq \theta$}
%             \Continue \Comment{Reject if context/time violates or PHI limit exceeded}
%         \EndIf
%         \If{\textbf{not} \Call{FulfillHardObligations}{$policy.\mathcal{B}_{\text{hard}}$}}
%             \State \Call{AuditLog}{$s, o, \text{"Hard obligation failed"}$}
%             \Continue \Comment{Deny if critical obligations (e.g., sanitization) fail}
%         \EndIf
%         \State \Call{FulfillSoftObligations}{$policy.\mathcal{B}_{\text{soft}}$} \Comment{e.g., Logging}
%         \State \Call{UpdateSession}{$S_t, o$} \Comment{Track PHI access count}
%         \State \Return \text{ALLOW} \Comment{First applicable policy grants access}
%     \EndFor
%     \State \Return \text{DENY} \Comment{Default deny}
% \EndFunction
% \end{algorithmic}
% \end{algorithm}\





% LLMs run on-premises model or APIs hosted by third parties operate as black-box models. To achieve continuous usage control, we interpose a middleware agent that intercepts requests/responses to/from the LLM. We track session-level information (e.g. user role, patient consent status, ongoing conversation context). If at any point the session attributes change (e.g., the user revokes consent mid-conversation), the policy engine reevaluates previously allowed data flows. Similarly, we also perform sequential query analysis because multi-turn conversations can lead to incremental disclosures of sensitive data. Our system maintains a short-term ``conversation state'' that updates after each LLM exchange. Policies can incorporate time-based or event-based conditions. For example, if user is requesting more than X pieces of PHI within a single session, raise an alert or re-verify authorization.


% The core of our methodology is a hybrid access control that unifies Role-Based Access Control (RBAC) and Attribute-Based Access Control (ABAC) using the usage control principles of the UCON$_{ABC}$ framework. This approach combines RBAC for static role hierarchies (e.g. role = cardiologist), ABAC for dynamic contextual attributes (e.g. data.sensitivity = PHI, time $\in$ [8 AM, 5 PM]), and UCON$_{ABC}$ for continuous authorization, obligations, and conditions checks. (e.g., logging) and mutability (e.g., revoking access mid-session).

% Authorization (A) rules integrate RBAC roles as immutable subject attributes and ABAC for environmental/time-sensitive conditions. Obligations (B) and Conditions (C) govern dynamic interactions during LLM workflows.




% The core of our methodology is based on the UCON$_{ABC}$ model, which provides a comprehensive approach to access control. 



% The Authorizations (A) module defines permission rules based on subject and object attributes, determining whether a particular user can access specific healthcare data. For example, a cardiologist (subject) with attribute ``role=cardiologist'' is authorized to query patient cardiac data (object) with attribute ``data\_type=cardiac'' but not psychiatric records. oBligations (B) specifies mandatory requirements that must be fulfilled before or during access, such as logging requirements or data anonymization procedures. For example, before accessing patient data, the system must log the access attempt, including user ID, timestamp, and access purpose. Additionally, the system must apply deidentification to any PHI before incorporating it into the prompts. Conditions (C) establish environmental or system-state prerequisites that must be satisfied, including time constraints, network security conditions, or system load factors. 

% To rigorously define policies, we model UCON\textsubscript{\textit{ABC}} components using \textbf{first-order logic}. Let:
% \begin{itemize}
%     \item \( S = \{s_1, \dots, s_n\} \) denote subjects (users) with attributes \( A_s = \{\text{role, clearance, department}\} \),
%     \item \( O = \{o_1, \dots, o_m\} \) denote objects (data/resources) with \( A_o = \{\text{sensitivity, type, owner}\} \),
%     \item \( C = \{c_1, \dots, c_k\} \) denote contextual conditions (time, network IP, consent status).
% \end{itemize}

% Authorization rules are expressed as:
% \begin{equation} \label{eq:authorization}
%     \text{Authorize}(s, o, \text{action}) \iff \bigwedge_{i} \phi_i(A_s, A_o, C),
% \end{equation}
% where \( \phi_i \) are predicates combining attributes and conditions. For instance:
% \begin{equation} \label{eq:predicate}
%     \phi_1: \text{role}(s) = \text{physician} \land \text{sensitivity}(o) \leq 2 \land \text{time} \in [8, 18].
% \end{equation}

% Obligations \( \mathcal{B} \) (e.g., logging, anonymization) are enforced as pre-conditions for authorization:
% \begin{equation} \label{eq:obligations}
%     \left(\bigwedge_{i} \phi_i(A_s, A_o, C)\right) \land \left(\mathcal{B} \text{ are fulfilled}\right) \implies \text{Authorize}(s, o, \text{action}),
% \end{equation}
% where \( \mathcal{B} = \{ \text{Log}(s, o, t), \text{Sanitize}(o) \} \).
% Policies are codified in an XACML-like syntax that maps directly to the formal model. For example, the rule for a cardiologist described above translates to Listing 1.
% \begin{lstlisting}[language=XML, caption={XACML-like policy for cardiologists}, label=lst:xacml]
% <Policy>
%   <Target>
%     <Subject>role=cardiologist</Subject>
%     <Resource>data_type=cardiac</Resource>
%   </Target>
%   <Condition>time E [8, 18]</Condition>
%   <Obligation>log_access</Obligation>
% </Policy>
% \end{lstlisting}
% The Policy Decision Point (PDP) evaluates these rules dynamically, incorporating real-time attributes (e.g., user role changes) and contextual shifts (e.g., consent revocation).


% Furthermore, we also sanitize the prompt in this step to ensure that LLMs do not can inadvertently memorize or regurgitate sensitive information. We refer to this as the pre-inference data sanitization step. Before the user asks or the LLM sends a request, the system attempts to identify the PHI. The sanitization pipeline uses a hybrid approach that includes regular expressions to match HIPAA-specified identifiers (SSN, MRN, phone numbers) for structured PHI detection and the BERT-based NER model fine-tuned on the MIMIC-IV (clinical notes) \cite{} dataset to detect contextual unstructured PHI (e.g. diagnoses, names). The identified PHI are then replaced with role-specific placeholders using a mapping function per privacy rules. For example, the input ``John Smith, born 5/5/1970, has diabetes. '' is sanitized and redacted to ``[PatientName], born [DOB], has diabetes.''


% \subsection {Policy Decision Agent}
% The PDP is responsible for evaluating access requests against predefined security and privacy policies. Acting as a decision-making engine, the PDP analyzes contextual attributes such as user roles, resource types, actions, and environmental conditions to determine whether access should be granted or denied. A high-level overview of the PDP algorithm is depicted in Algorithm \ref{algo_1}  where chkCtxCond is CheckContextualConditions, and matchAttr is MatchAttributes. 

% \begin{algorithm}
% \caption{UCON$_{ABC}$ Policy Decision Point}
% \label{algo_1}
% \begin{algorithmic}[1]
% \Function{EvaluateRequest}{$s, o, action, context$}
%     \State $policies \gets \text{LoadPolicies}()$
%     \For{$policy \in policies$}
%         \If{$\text{matchAttr}(s, o, policy.conditions)$}
%             \If{$\text{chkCtxCond}(context, policy.conditions)$}
%                 \If{$\text{FulfillObligations}(policy.obligations)$}
%                     \State \Return $Decision.ALLOW$
%                 \EndIf
%             \EndIf
%         \EndIf
%     \EndFor
%     \State \Return $Decision.DENY$
% \EndFunction
% \end{algorithmic}
% \end{algorithm}




%  Traditional access control models (for example, RBAC, ABAC) typically grant or deny access to data based on policies evaluated at the moment of request. In contrast, UCON$_{ABC}$ focuses on mutable attributes and continuous policy evaluation, including obligations and conditions that persist over time \cite{sandhu2003usage}. This continuous enforcement is crucial for LLMs, as repeated queries over the same data could lead to progressive disclosures. Moreover, LLMs do not ``forget'' internal representations easily and can generate text referencing prior sessions or hidden embeddings. 
% There are eight core components in the UCON$_{ABC}$ model such as \textit{subjects, subject attributes, objects, object
% attributes, rights, authorizations, obligations,} and
% \textit{conditions} (see Figure \ref{fig: usage_control}). 
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale=1.10]{figs/HIPPA LLM - Page 4-1.pdf}
%     \caption{ABC Model Components. Adapted from \cite{sandhu2003usage}.}
%         \label{fig: usage_control}
% \end{figure} 


% The subjects and objects align with traditional access control concepts. The attributes of the subjects include factors such as identity, role, group membership, and security clearance, while objects represent the resources with which the subjects can interact.  For example, in the healthcare ecosystem, the clinician, the administrator, and the patient can be subject. The patient's medical records are objects. A right grants a subject permission to access an object in a specific manner, such as reading or modifying data. 

% Authorization, obligations, and conditions are key elements in usage control decisions. Authorization rules determine whether a subject is allowed or denied access to an object based on their respective attributes. Obligations refer to specific actions that must be carried out by the subject or the system before access is granted. Conditions are external factors or system constraints that influence access permissions.

% The authorization, obligations,
% and conditions are components of usage control decisions. The authorization rule
% permits or denies the access of a subject to an object
% based on subject and object attributes. Obligations are
% performed by subjects or by the system. Conditions are
% system environment restrictions. In the usage control
% model, subjects and objects are familiar concepts with
% traditional access control. Subject and object attributes
% can be used during the access decision process. Subject
% attributes are identities, group names, roles, memberships,
% security clearance, and so on. Objects are entities that
% subjects hold rights on, whereby the subjects can access
% or use objects. For instance, in an e-Healthcare system,
% doctors, nurses and physicians can be subject. A patient’s
% medical records are objects. Rights are privileges that
% subjects can hold on objects. The authorizations of rights
% require associations with subjects and objects. 

% A right

% represents the access of a subject to an object, such as
% read or write.
% Authorizations, obligations and conditions are decision
% factors used to check and determine whether a subject
% should be allowed to access an object. Obligations and
% conditions are new concepts that can resolve certain
% shortcomings that have been in traditional access controls.
% In general, the authorization of most traditional access
% controls are assumed to be done before access is allowed.
% However in the usage control model it extends this for
% continuous enforcement. Authorizations may require
% updates on subject and object attributes. The process of
% continuity properties in usage control model consists of
% three phrases, before usage, ongoing usage and after
% usage. To enforce control decisions, we have two
% different types: pre-decision and ongoing-decision. For
% mutability, there are three kinds of updates: pre-update,
% ongoing-update, and post-update. Therefore,
% Authorizations can be either pre-authorization (preA) or
% ongoing-authorization (onA). Pre-authorization is
% performed before authorization is required to the access.
% But ongoing authorization may be performed during the
% access, such as when a patient medical record in a
% hospital is periodically checked while the access is in
% progress.








 
% 2.3 Challenges

%     Policy Granularity: HIPAA rules often require extremely fine-grained control (e.g., partial data sharing or selective field redaction). Implementing these at scale in dynamic user interactions is non-trivial.
%     Black-Box Inference: Most LLMs are developed by third parties who do not disclose model internals, complicating efforts to log or intercept sensitive data usage.
%     Contextual Leaks: The model might generate responses that are not explicitly labeled as PHI but still allow an informed adversary to infer sensitive details.
%     Traceability and Auditing: Proper compliance requires an audit trail. Retrofitting LLMs with continuous logs of context, queries, and partial model states is currently an open research question.


%\cite{hastings2024preventing}.

%The integration of LLM is poised to transform healthcare delivery through improved diagnostic and operational capabilities \cite{clusmann2023future}. This integration offers benefits to both healthcare providers and patients. For example, automatic generation of clinical summaries can alleviate the administrative burden of updating the EHR, a task strongly associated with physician burnout \cite{knoll2022user} . On the other hand, for patients, these summaries can also improve patient understanding of post hospitalization careplans and reduce the risk of misinterpretation of medical information \cite{10825266}. Similarly, context-augmentation frameworks for medical question-answering, such as MedInsight \cite{10.1145/3709365}, provide personalized, targeted, and contextually relevant medical recommendations utilizing patient medical history and trusted authoritative medical knowledge. Such frameworks empower patients and caregivers with the information necessary to improve self-care, improve patient care, and optimize healthcare outcomes.

% Despite rapid advancements in the technical sophistication of these systems, it is crucial to be aware of fundamental limitations as well as technical and regulatory challenges \cite{hastings2024preventing}. These concerns require the development of structured implementation protocols that align advanced analytics with established patient privacy protections (e.g. HIPAA compliance) while maintaining accountability in automated care pathways.



%employs autonomous, specialized agents governed by Attribute-Based Access Control (ABAC) (\S\ 164.312(a)(1)) and layered PHI sanitization (\S\ 164.514(b)(2)) mechanisms to enforce least-privilege data access, redact sensitive information at multiple pipeline stages, and maintain immutable audit trails (\S\ 164.312 (b)). 






% Unlike static frameworks, our UCON$_{ABC}$ implementation continuously evaluates contextual factors (e.g., user role, data sensitivity, LLM task legitimacy) and enforces obligations (e.g., real-time redaction, audit logging) to protect PHI. 


% The architecture integrates Policy Decision Points (PDP), Policy Enforcement Points (PEP), and specialized middleware agents to enable continuous policy evaluation, pre-inference sanitization, and post-inference redaction. By implementing these dynamic authorization controls throughout the processing pipeline, our solution ensures PHI remains accessible only to intended users while enabling healthcare organizations to safely leverage LLM capabilities at scale, establishing a foundation for HIPAA-compliant, responsible AI adoption in clinical settings.


% In an informal user study (N=5) with clinicians and administrative staff, we simulated real-world queries:

%     Single-Query Scenario: A doctor asked for a summary of a fictitious patient’s symptoms. Our policy engine successfully removed personally identifying attributes while retaining relevant clinical details.
%     Multi-Query Scenario: Repeated questions by an administrative user included partial references to the patient’s identity. After several consecutive queries, our classifier flagged attempts to infer the patient’s identity from previously redacted placeholders, but false positives also rose—sometimes blocking legitimate follow-up questions.

% Lessons Learned:

%     Tradeoff Between Context Preservation and Privacy: Overzealous redaction can limit the model’s utility.
%     Need for Context-Aware Policies: A static policy approach struggles to track partial disclosures across multiple queries.
%     Computational Overhead: On-the-fly scanning and redaction introduce latency, which might be critical in real-time healthcare applications.


logging with three key features:

% \begin{itemize}
%     \item \textbf{Attribute-Centric Logging}: Structured records contain:
%     \begin{lstlisting}[language=json]
% {
%   "timestamp": "2023-10-05T14:30Z",
%   "subject": {"role": "radiologist", "department": "imaging"},
%   "resource": {"type": "CT_scan", "sensitivity": 3},
%   "action": "generate_report",
%   "environment": {"network": "hospital_lan", "consent": "valid"},
%   "decision": "ALLOW",
%   "obligations": ["REDACT_DEMO", "LOG_FULL"]
% }
%     \end{lstlisting}

%     \item \textbf{Immutable Evidence Chain}:
%     \begin{itemize}
%         \item Cryptographic hash linking: 
%         \begin{equation}
%             H_{n} = \text{SHA3}(H_{n-1} \parallel \mathit{log\_entry}_n)
%         \end{equation}
%         \item WORM (Write-Once-Read-Many) storage for raw LLM outputs
        
%     \end{itemize}

%     \item \textbf{Real-Time Anomaly Detection}:
%     \begin{equation}
%         \mathit{alert} = 
%         \begin{cases}
%             1 & \text{if } \mathit{access\_rate}(u) > 3\sigma \\
%             1 & \text{if } \Delta\mathit{phi\_accessed} > \mathit{threshold} \\
%             0 & \text{otherwise}
%         \end{cases}
%     \end{equation}
%     Triggers MFA reauthentication when $\mathit{alert}=1$.
% \end{itemize}
% \begin{equation*}
% \small
% \phi_1: \text{role}(s) = \text{physician} \land \text{sensitivity}(o) \leq 2 \land \text{action}(a) = \text{read} \land \text{time}(e) \in [8, 18].
% \end{equation*}
